Radio Loud vs. Radio Quiet Gamma-ray Bursts: the Role of Binary Progenitors

We explore the possibility that radio loud gamma-ray bursts (GRBs) result from the collapse of massive stars in interacting binary systems, while radio quiet GRBs are produced by the collapse of single massive stars. A binary collapsar system can have the necessary angular momentum and energy budget to explain the longer prompt gamma-ray durations and higher isotropic energies seen in the the radio loud sub-sample of long GRBs. Additionally binary systems can lead to rich and extended circumstellar environments that allow for the presence of the long-lived radio afterglows seen in the radio loud systems. Finally, the relative fraction of stars in binary systems versus single star systems appears consistent with the fraction of radio loud versus radio quiet GRBs.

==> Makefile <==
LATEXMK=latexmk

SRC=header.tex \
    main.bib 

default: bhns

all: bhns

bhns: main.pdf

%.pdf: %.tex ${SRC} $(shell find figures/)
	${LATEXMK} -f -pdf $<

clean:
	rm -f ./*.aux ./*.bbl ./*.blg ./*.log ./*.nav ./*.out ./*.snm ./*.toc ./*.fls ./*.fdb_latexmk mainNotes.bib main.pdf


